Higgs Assisted Razor Search for Higgsinos at a 100 TeV pp Collider

A 100 TeV proton-proton collider will be an extremely effective way to probe the electroweak sector of the Minimal Supersymmetric Standard Model (MSSM). In this paper, we describe a search strategy for discovering pair-produced Higgsino-like next-to-lightest supersymmetric particles (NLSPs) at a 100 TeV hadron collider that decay to Bino-like lightest supersymmetric particle (LSP) via intermediate Z and SM Higgs boson that in turn decay to a pair of leptons and a pair of b-quarks respectively: $\widetilde{N}_2^0\widetilde{N}_3^0 \rightarrow (Z\widetilde{N}_1^0)(h\widetilde{N}_1^0)\rightarrow bb\ell\ell+\widetilde{N}_1^0\widetilde{N}_1^0$. In addition, we examine the potential for machine learning techniques to boost the power of our searches. Using this analysis, Higgsinos up to 1.4 TeV can be discovered at $5\sigma$ level for a Bino with mass of about 0.9 TeV using 3000 fb$^{-1}$ of data. Additionally, Higgsinos up to 1.8 TeV can be excluded at 95% C.L. for Binos with mass of about 1.4 TeV. This search channel extends the multi-lepton search limits, especially in the region where the mass difference between the Higgsino NLSPs and the Bino LSP is small.

==> tables/3attobarns_events_table.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} &   Signal &        tt &       tbW &    bg_tot &       S/B &  Significance \\
\midrule
Original            &  1002.59 &  1.08e+08 &  1.25e+07 &  1.21e+08 &  8.32e-06 &          0.09 \\
At least one lepton &   903.65 &  1.06e+08 &  1.12e+07 &  1.17e+08 &  7.71e-06 &          0.08 \\
Lepton trigger      &   845.96 &  1.59e+07 &  2.74e+06 &  1.87e+07 &  4.54e-05 &          0.20 \\
2 leptons           &   688.72 &  1.07e+07 &  1.42e+06 &  1.21e+07 &  5.70e-05 &          0.20 \\
SF leptons          &   685.92 &  5.36e+06 &  7.17e+05 &  6.07e+06 &  1.13e-04 &          0.28 \\
OS leptons          &   684.75 &  5.28e+06 &  7.17e+05 &  6.00e+06 &  1.14e-04 &          0.28 \\
2 b jets            &   108.65 &  7.68e+05 &  1.45e+05 &  9.13e+05 &  1.19e-04 &          0.11 \\
MET                 &    76.57 &  1.29e+04 &  1.18e+04 &  2.46e+04 &  3.11e-03 &          0.49 \\
m_ll                &    63.59 &  4.93e+03 &  5.83e+03 &  1.08e+04 &  5.91e-03 &          0.61 \\
m_bb                &    56.86 &  1.49e+03 &  4.70e+02 &  1.96e+03 &  2.90e-02 &          1.28 \\
m_R                 &    50.11 &  7.14e+01 &  7.34e+01 &  1.45e+02 &  3.46e-01 &          4.16 \\
mTR                 &    49.90 &  2.38e+01 &  4.40e+01 &  6.78e+01 &  7.36e-01 &          6.06 \\
\bottomrule
\end{tabular}


==> tables/mc_events_table.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Signal &        tt &     tbW \\
\midrule
Original            &  905000 &  13613911 &  853700 \\
At least one lepton &  815696 &  13373983 &  762203 \\
Lepton trigger      &  763619 &   2005571 &  186833 \\
2 leptons           &  621686 &   1344918 &   97024 \\
SF leptons          &  619153 &    675419 &   48867 \\
OS leptons          &  618098 &    666185 &   48862 \\
2 b jets            &   98073 &     96865 &    9860 \\
MET                 &   69120 &      1622 &     803 \\
m_ll                &   57397 &       622 &     397 \\
m_bb                &   51324 &       188 &      32 \\
m_R                 &   45232 &         9 &       5 \\
mTR                 &   45046 &         3 &       3 \\
\bottomrule
\end{tabular}

